Automated Repair of Ambiguous Problem Descriptions for LLM-Based Code Generation

The growing use of large language models (LLMs) has increased the importance of natural language (NL) in software engineering. However, ambiguity of NL can harm software quality, as unclear problem descriptions may lead to incorrect program generation. Detecting and resolving such ambiguity is challenging, motivating our introduction of the automated repair of ambiguous NL descriptions, which we approach by reducing code generation uncertainty and better aligning NL with input-output examples. Ambiguity repair is difficult for LLMs because they must understand how their interpretation of a description changes when the text is altered. We find that directly prompting LLMs to clarify ambiguity often produces irrelevant or inconsistent edits. To address this, we decompose this task into two simpler steps: (1) analyzing and repairing the LLM's interpretation of the description - captured by the distribution of programs it induces - using traditional testing and program repair, and (2) refining the description based on distribution changes via a method we call contrastive specification inference. We implement this approach in a tool called SpecFix and evaluate it using four state-of-the-art LLMs (GPT-4o, GPT-4o-mini, DeepSeek-V3, and Qwen2.5-Coder-32B-Instruct) on three popular code generation benchmarks (HumanEval+, MBPP+ and LiveCodeBench). Without human intervention or external information, SpecFix modified 43.58% of descriptions, improving Pass@1 on the modified set by 30.9%. This yields a 4.09% absolute improvement across the entire benchmark. Repairs also transfer across models: descriptions repaired for one model improve other models' performance by 10.48%.

==> sections/specfix.tex <==
\section{SpecFix}
\label{sec:specfix}

\subsection{Specification Repair Problem}

The repair problem introduced in this work is defined as follows:

\begin{definition}
Let $R\in\mathcal{R}^{\smiley}$ be a natural language specification, and $\phi$ be a quality criteria such that $\neg\phi(R)$. The goal of specification repair is to find a modification $R'\in\mathcal{R}^{\smiley}$ such that $\phi(R)$.
\end{definition}

There are two key elements of this definition, the quality criteria $\phi$ and the set of ``good'' requirements $R\in\mathcal{R}^{\smiley}$.

For ambiguous specifications when we do not know the exact expected program behavior, the quality criterion is defined via the measure from previous work shown in \Cref{eq:ambiguity}: $$\phi_\mathrm{unambiguous}{}(R) \triangleq \mathrm{ambiguity}(R) < \tau \quad \text{for some }\tau.$$ When using this criterion, it is appropriate to generate multiple possible repairs and ask the user to select their preferred variant.

For ambiguous or incorrect specifications, when the expected semantics is given in the form of a program $P$, we define the \emph{$P$-consistency} requirement: $$\phi_{P-\mathrm{consistent}}(R) \triangleq \hat{m}_\equiv([P], R) > \tau \quad \text{for some }\tau.$$ This criterion is applicable, for example, when software evolution causes a code-comment inconsistency, and an outdated comment is repaired based on the evolved code.

For ambiguous or incorrect specifications, when the expected semantics is given in the form of tests $T$, we define the \emph{$T$-consistency} requirement: $$\phi_{T-\mathrm{consistent}}(R) \triangleq \left(\sum_{P \text{ passes }T} \hat{m}(P, R) \right)> \tau \quad \text{for some }\tau.$$

The above definitions imply that we are able to compute $\hat{m}_\equiv$ and therefore assume at least the realizability of the requirements (\Cref{eq:realizable}). \sergey{this is not logical}. This might happen for at least two reasons: (1) an LLM is not capable to realize the requirements, or (2) the requirements are so high-level that the desired implementation does not appear in  $\hat{m}_\equiv$. For example, consider the following requirements: ``the program returns a positive number''. Even though the program that computes the $n-$th Catalan number satisfies this requirement, and can be realised by an LLM, and it unlikely to appear in $\hat{m}_\equiv$.

\subsection{Example of Ambiguous Specification}

Consider the specification $R$ in \Cref{eq:sort_while_removing}. It is ambiguous because it does not make it clear if the duplicates need to be removed before or after sorting. When GPT-4o, a SOTA LLM, was prompted to clarify the requirements, it asked eight clarification questions, involving ``Should elements be considered consecutive duplicates only if they are directly adjacent in the array, or do duplicates elsewhere in the array count as well?'' However, ``consecutive duplicates'' is arguably not an ambiguous formulation, and the probability of GPT-4o's generating a program with an alternative interpretation of this requirement is diminishingly low. This shows that directly asking an LLM to assess if requirements are ambiguous is suboptimal, since it may generate irrelevant clarification requests. 

To make ambiguity detection more precise, we propose a reflection-based mechanism, where an LLM is first tasked with generating a program $P$ based on the requirement $R_2$, and then asked to produce new requirements $R_3$ of $P$ via code summarization~\cite{ahmed2022few}. Since $P$ inevitably defines a specific order of operations, this order will be reflected in $R_3$.\haoxiang{Sometime not. The  requirement may still implicitly describe the order.} Then, by comparing $\mathrm{DRS}(R_2)$ and $\mathrm{DRS}(R_3)$, we identify discrepancies such as that $R_3$ involves an additional predicate on the sequence of events \(t_1 < t_2\).

A limitation of this approach is that some of the clarifying question might be redundant. Consider, for example, the following requirements:
\begin{equation*}
\begin{split}
R_4 \triangleq ``&\text{Implement a function that sorts a given array}\\[-0.3em]
&\text{while removing zeros.}"   
\end{split}
\end{equation*}
Although it has the same ambiguity as $R_2$, changing the order of operations will not affect the outcome. Therefore, clarifying this requirement is counterproductive. To address this issue, we define a measure of semantic divergence between requirements:
\[
\mathrm{divergence}(R_1, R_2) \triangleq d(m_\equiv(\cdot \mid R_1), m_\equiv(\cdot \mid R_2)).
\]
As with \Cref{eq:ambiguity}, this divergence can be estimated through sampling and differential testing.

Assume that $R$ are the initial requirements, and requirements $R'$ are obtained through our reflection mechanism such as $\mathrm{DRS}(R')$ differ from $\mathrm{DRS}(R)$ by an extra proposition $\phi$. Then, we only ask the user to clarify $R$ wrt $\phi$ if there is a significant divergence between $R \wedge \phi$ and $R \wedge \neg\phi$. This allows avoiding redundant clarifications.

\subsection{Sometimes Ambiguity is Not an Issue}

There are situations when the problem naturally accepts multiple semantically diverging solutions. Consider the following requirements:
\begin{equation*}
\begin{split}
R_5 \triangleq ``&\text{prints all positive numbers}\\[-0.3em]
&\text{stored in the nodes of a graph.}"   
\end{split}
\end{equation*}
The order of printed numbers depends on the chosen graph traversal order, e.g. DFS or BFS. However, this order may not be important for the user. Internally the system will store an arbitrary clarification of these requirements to ensure convergence of the elicitation process.

